CALM: Cognitive Assessment using Light-insensitive Model

The demand for cognitive load assessment with low-cost easy-to-use equipment is increasing, with applications ranging from safety-critical industries to entertainment. Though pupillometry is an attractive solution for cognitive load estimation in such applications, its sensitivity to light makes it less robust under varying lighting conditions. Multimodal data acquisition provides a viable alternative, where pupillometry is combined with electrocardiography (ECG) or electroencephalography (EEG). In this work, we study the sensitivity of pupillometry-based cognitive load estimation to light. By collecting heart rate variability (HRV) data during the same experimental sessions, we analyze how the multimodal data reduces this sensitivity and increases robustness to light conditions. In addition to this, we compared the performance in multimodal settings using the HRV data obtained from low-cost fitness-grade equipment to that from clinical-grade equipment by synchronously collecting data from both devices for all task conditions. Our results indicate that multimodal data improves the robustness of cognitive load estimation under changes in light conditions and improves the accuracy by more than 20% points over assessment based on pupillometry alone. In addition to that, the fitness grade device is observed to be a potential alternative to the clinical grade one, even in controlled laboratory settings.

==> Chapters/2-RelatedWorks.tex <==
Tremendous efforts were invested in cognitive load assessment from ECG and pupillometry data. Our work leverages the most recent feature extraction and analysis techniques.

\subsection{Pupillometry}

The variation of the pupil diameter when performing a task is widely used as a cognitive load estimator. Comparison of the cognitive load estimation results from gaze tracking and pupillary response identified the benefits of both eye movement-based measures \cite{pd_gaze_cogload-Krejtz-2018}. Even though it is among the most recent quantitative cognitive metrics, pupillometry accounts for a significant amount of research \cite{pupil_cogload-Weber-2021, PupillometryPP-Matht-2018}. The pioneering work of Murata et al. \cite{Murata1998} investigated the rhythmic fluctuations in pupil diameter for evaluating mental load, concluding that it can be as effective as HRV. The utility of pupillometry as a mental load estimator stems from the pupil's sensitivity to physiological factors related to the autonomic nervous system (ANS). %The ANS oversees involuntary body functions, including breathing, pupil response, and heart activity.
Various hand-crafted features were devised to capture the cognitive load variation from pupillometry. The most common features for pupillometry in cognitive load research are mean pupil diameter, standard deviation of the pupil diameter, Index of Pupillary Activity (IPA), Pupil AUC (Area Under the Curve), and PDRoC (Pupil Diameter Rate of Change).

%Many diverse applications benefit from using pupil diameter measurements. For instance, in \cite{Eckert2022}, researchers studied the effect of pupil diameter changes in response to light reflex to optimize virtual reality experiences. Additionally, pupillometry can differentiate dementia-related illnesses. In \cite{Mohamad2022}, the change in pupil diameter induced by cognitive load was investigated in both dementia patients and healthy individuals to differentiate them. Human-computer interaction (HCI) has also benefited significantly from pupillometry \cite{hci_pupil-mathot-2016}, using it to evaluate the cognitive demands of user interfaces and adaptive systems.  

One of the main drawbacks of pupillometry is that pupil diameter changes according to external light conditions. This means that features derived from pupil diameter are influenced not only by cognitive load but also by ambient light. To mitigate this sensitivity, Duchowski et al. developed the Index of Pupillary Activity (IPA) and the Low/High Index of Pupillary Activity (LHIPA) features \cite{Duchowski2018, Duchowski2020}. The Index of Cognitive Activity (ICA) is also widely recognized as less sensitive to light \cite{ica-Marshall-2002}. However, many recent studies have observed that these features still suffer from variations in light conditions \cite{light_compare-Nickolas-2024}. Our experiments also confirmed the sensitivity of pupillometry-derived features to ambient light, leading us to adopt a multimodal approach to reduce this sensitivity. %Recently, multimodal data acquisition has gained popularity, as complementary features from multiple sensors can provide more reliable and robust cognitive load estimates \cite{multimodal_cogload-Vanneste-2020, multi_modal_CogLoad-Kim-2021}. 


\subsection{Heart rate Variability}
Heart rate variability (HRV) \cite{hrv_old-MESHKATI-1988} is one of the most popular and commonly used measures of cognitive load due to its well-established methodology in the medical domain. Additionally, HRV is relatively robust to most external influences and is easy to measure and post-process. This measure is favored because of its direct relation to the ANS. The interaction between the sympathetic and parasympathetic nervous systems, the two main components of the ANS, is identified in heart activity as low-frequency (LF) and high-frequency (HF) bands. The balance between these two frequencies, known as the sympathovagal balance, is directly related to cognitive load \cite{hrv_sympathovogal-Kathrin-2021}.

The primary source of noise in this mental workload measure is the effect of breathing. The study presented in \cite{Lenis2017} addresses this issue, noting that not accounting for the breathing effect could lead to incorrect diagnoses. Many applications, such as the work by Kavousi \cite{Kavousi2022}, demonstrate the utility of measuring cognitive load from HRV to estimate the state and stress levels of novice car drivers, enabling adaptive system responses. In \cite{hrv_covid-Aristizabal-2020}, Aristizabal et al. proposed monitoring the stress levels of frontline healthcare workers by tracking their HRV during COVID-19 interventions. In educational settings, HRV is used to assess the cognitive load, providing insights into student engagement and learning effectiveness \cite{hrv_edu-Park-2022}.

%The main objective of using HRV in our study is to complement pupillometry, which is sensitive to changes in light conditions. We established multimodal data acquisition settings that integrate both pupillometry and HRV to provide a more robust assessment of cognitive load.

%We also compared using any single modality is better than using both modalities. As for the HRV data acquisition, we also compared two popular devices, Polar H10 and Biopac MP35. Polar H10 is a wireless fitness grade equipment suitable for activity tracking. Biopac MP35 is an accurate high-fidelity clinical grade equipment used primarily in laboratory settings. It is wired, thus restricting the mobility of the participants during the data acquisition phase. The objective of this comparison was to verify whether low-cost fitness grade equipment is enough for accurately estimating cognitive load, especially when the subject can be moving during data acquisition.

\subsection{Feature Extraction and Classification}
Hand-crafted features are widely used in the feature extraction stages in most cognitive load estimation works \cite{MAUS_dataset-Beh-2021, Albuquerque2020, light_compare-Nickolas-2024}. As the application requirements diversify further, new features are created to meet the requirements such as real-time extraction \cite{ica-Marshall-2002} and robustness in the wild \cite{cogload_wild-Fridman-2018}, among many others. Due to the relatively low availability of data for targeted behavioral studies (typically the number of participants is less than 20 and the session length is less than 10 minutes), feature learning using modern deep learning techniques is not easy to adapt to this type of setting \cite{nn_sampling-Meethal-2022}.
%However, our experimental results show comparable results to the hand-crafted features in many settings using the transformer-based models \cite{transformer-Vaswani-2017}.
Among the most common features derived from HRV are RMSSD (Root Mean Square of Successive interval Differences.), SDNN (Standard Deviation of Normal-to-Normal Interbeat Intervals.), pNN50 (Proportion of NN50; NN50 is the number of pairs of successive NN intervals that differ by more than 50 ms), Mean RR interval (average time between successive heartbeats), Median RR interval (median duration between successive heartbeats), Respiration Rate, HF (High Frequency, ie the frequency band between 0.15 and 0.40 Hz), and LFHF Ratio (ratio of power in Low Frequency (LF) band to the power in the HF band). More details about these features are available in \cite{hrv_features-Fred-2017}. %Additional details about these features will be discussed in the next section. We used sliding windows during feature extraction to increase the number of datapoints.

The classification methods employed in most of the previous contributions are derived from classical machine learning techniques. Random Forest and Support Vector Machines (SVMs) are widely used with hand-crafted features \cite{Dengbo2022, Mitre2022, Albuquerque2020}. We believe they lack comparison with a multi-layer neural network (utilizing hand-crafted features) and more recent approaches such as transformer-based classifiers (which use learnable features from the 1D signal). %Additional details about the architecture of the two models are provided in the appendix. 

==> Chapters/6-DL.tex <==


